Fast and Flexible Bayesian Inference in Time-varying Parameter Regression Models

In this paper, we write the time-varying parameter (TVP) regression model involving K explanatory variables and T observations as a constant coefficient regression model with KT explanatory variables. In contrast with much of the existing literature which assumes coefficients to evolve according to a random walk, a hierarchical mixture model on the TVPs is introduced. The resulting model closely mimics a random coefficients specification which groups the TVPs into several regimes. These flexible mixtures allow for TVPs that feature a small, moderate or large number of structural breaks. We develop computationally efficient Bayesian econometric methods based on the singular value decomposition of the KT regressors. In artificial data, we find our methods to be accurate and much faster than standard approaches in terms of computation time. In an empirical exercise involving inflation forecasting using a large number of predictors, we find our models to forecast better than alternative approaches and document different patterns of parameter change than are found with approaches which assume random walk evolution of parameters.

==> Tables/old/best_forecast.tex <==
%latex.default(full.table, file = paste0(dir, "/", "BF_scores_RWbench.tex"),     title = "", ctable = FALSE, rgroupTexCmd = "scshape", n.cgroup = n.cgroup,     cgroup = cgroup, rgroup = rgroup, n.rgroup = n.rgroup, caption = "Bayes factors relative to RW-SV. ***, **, and * refer to signficance at the 1%, 5% and 10% level according to the DM (AG) test statistic.",     label = "tab:LPS", size = "tiny", booktabs = TRUE, rowname = "",     colheads = NULL, numeric.dollar = FALSE, caption.loc = "bottom",     landscape = FALSE)%
\begin{table}[t]
{\tiny
\begin{center}
\caption{\label{tab:LPS} Forecasting Performance of SVD Approaches Relative to Benchmarks}
\begin{tabular}{llllcll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{3}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{2}{c}{\bfseries Forecast horizon}\tabularnewline
\cmidrule{2-4} \cmidrule{6-7}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{TVP/TIV}&\multicolumn{1}{c}{Type}&\multicolumn{1}{c}{$\kappa$}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{1-step}&\multicolumn{1}{c}{4-steps}\tabularnewline
\midrule
{\scshape AR(p)}&&&&&&\tabularnewline
~~&TIV&Benchmark&&&0.90&0.77***\tabularnewline
~~&&&&&(0.08)&(0.23***)\tabularnewline
~~&TVP-FFBS-RW&Benchmark&&&0.90&0.75***\tabularnewline
~~&&&&&(0.08)&(0.26***)\tabularnewline
\midrule
{\scshape FULL}&&&&&&\tabularnewline
~~&TIV&Benchmark&&&0.82*&0.61**\tabularnewline
~~&&&&&(0.15)&(0.37)\tabularnewline
~~&TVP-FFBS-fac&Benchmark&&&0.83**&0.63\tabularnewline
~~&&&&&(0.17**)&(0.25)\tabularnewline
~~&TVP-FFBS-RW&Benchmark&&&0.78*&0.92\tabularnewline
~~&&&&&(0.16)&(0.01)\tabularnewline
\cmidrule{2-7}
~~&TVP-SVD&g-prior&0.1&&0.80***&0.59**\tabularnewline
~~&&&&&(0.15**)&(0.42*)\tabularnewline
~~&TVP-SVD&g-prior (clustering)&0.05&&0.80***&0.57***\tabularnewline
~~&&&&&(0.17**)&(0.48***)\tabularnewline
~~&TVP-SVD&Minnesota&0.1&&0.82**&0.61**\tabularnewline
~~&&&&&(0.16*)&(0.37*)\tabularnewline
\midrule
{\scshape NKPC}&&&&&&\tabularnewline
~~&TIV&Benchmark&&&0.91&0.82***\tabularnewline
~~&&&&&(0.06)&(0.12)\tabularnewline
~~&TVP-FFBS-RW&Benchmark&&&0.92&0.86\tabularnewline
~~&&&&&(0.07)&(-0.28*)\tabularnewline
\cmidrule{2-7}
~~&TVP-SVD&g&0.001&&0.89&0.79***\tabularnewline
~~&&&&&(0.07)&(0.13)\tabularnewline
~~&TVP-SVD&g-prior (clustering)&0.001&&0.90&0.80***\tabularnewline
~~&&&&&(0.07)&(0.12)\tabularnewline
~~&TVP-SVD&Minnesota&0.001&&0.91&0.81***\tabularnewline
~~&&&&&(0.05)&(0.13)\tabularnewline
\midrule
{\scshape PCA3}&&&&&&\tabularnewline
~~&TIV&Benchmark&&&0.92&0.83***\tabularnewline
~~&&&&&(0.06)&(0.18***)\tabularnewline
~~&TVP-FFBS-RW&Benchmark&&&0.88&0.86\tabularnewline
~~&&&&&(0.09)&(0.05)\tabularnewline
\midrule
{\scshape TARP}&&&&&&\tabularnewline
~~&TIV&Benchmark&&&0.99&0.85***\tabularnewline
~~&&&&&(0.01)&(0.15***)\tabularnewline
~~&TVP-FFBS-RW&Benchmark&&&0.92***&0.82\tabularnewline
~~&&&&&(0.14***)&(0.17)\tabularnewline
\midrule
{\scshape UCM}&&&&&&\tabularnewline
~~&TVP-FFBS-RW&Benchmark&&&0.86***&0.59**\tabularnewline
~~&&&&&(0.16)&(0.16)\tabularnewline
~~&TVP-SVD&g-prior (clustering)&1&&0.88*&0.71\tabularnewline
~~&&&&&(0.08)&(0.14)\tabularnewline
\bottomrule
\end{tabular}
%\caption{}\end{center}}
\end{center}}
\begin{minipage}[c]{\linewidth}
\footnotesize{\textbf{Notes}: The table shows RMSEs with LPL's in parentheses below. Asterisks indicate statistical significance for each model relative to a random walk at the $1$ ($^{***}$), $5$ ($^{**}$) and $10$ ($^{*}$) percent significance levels. }
\end{minipage}
\end{table}


==> Tables/old/svd_forecast.tex <==
%latex.default(table.svd, file = paste0(dir, "/", "svd_forecast.tex"),     title = "", ctable = FALSE, rgroupTexCmd = "scshape", n.cgroup = n.cgroup,     cgroup = cgroup, rgroup = rgroup, n.rgroup = n.rgroup, caption = "",     label = "tab:LPS", size = "tiny", booktabs = TRUE, rowname = "",     colheads = colheads, numeric.dollar = FALSE, caption.loc = "bottom",     landscape = FALSE)%
\begin{table}[!tbp]
{\tiny
\begin{center}
\caption{Forecasting Performance for Different Values of $\kappa$ \label{tab:LPS1}}
\begin{tabular}{lllcllllll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{2}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{6}{c}{\bfseries $\kappa$}\tabularnewline
\cmidrule{2-3} \cmidrule{5-10}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{Horizon}&\multicolumn{1}{c}{Information set}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{0.001}&\multicolumn{1}{c}{0.005}&\multicolumn{1}{c}{0.01}&\multicolumn{1}{c}{0.05}&\multicolumn{1}{c}{0.1}&\multicolumn{1}{c}{1}\tabularnewline
\midrule
{\scshape g-prior (no clustering)}&&&&&&&&&\tabularnewline
~~&1-step-ahead&FULL&&0.81**&0.82**&0.80**&0.79***&0.80***&\tabularnewline
~~&&&&(0.15*)&(0.12)&(0.18**)&(0.13)&(0.15**)&\tabularnewline
~~&&NKPC&&0.89&0.88&0.89&0.94&1.02&\tabularnewline
~~&&&&(0.07)&(0.06)&(0.00)&(-0.07)&(-0.15**)&\tabularnewline
~~&4-step-ahead&FULL&&0.60**&0.59**&0.61**&0.58**&0.59**&\tabularnewline
~~&&&&(0.35)&(0.36)&(0.35)&(0.41*)&(0.42*)&\tabularnewline
~~&&NKPC&&0.79***&0.78*&0.76*&0.85&0.95&\tabularnewline
~~&&&&(0.13)&(0.11)&(0.10)&(0.03)&(-0.03)&\tabularnewline
\midrule
{\scshape g-prior (clustering)}&&&&&&&&&\tabularnewline
~~&1-step-ahead&FULL&&0.82**&0.81**&0.80***&0.80***&0.76**&\tabularnewline
~~&&&&(0.16*)&(0.13)&(0.15*)&(0.17**)&(0.13)&\tabularnewline
~~&&NKPC&&0.90&0.88*&0.88*&0.96&1.31&\tabularnewline
~~&&&&(0.07)&(0.00)&(-0.05)&(-0.14*)&(-0.24***)&\tabularnewline
~~&&UCM &&1.10**&1.10**&1.11**&1.05&1.01&0.88*\tabularnewline
~~&&&&(-0.26***)&(-0.26***)&(-0.25**)&(-0.19**)&(-0.18*)&(0.08)\tabularnewline
~~&4-step-ahead&FULL&&0.60***&0.60***&0.59***&0.57***&0.69**&\tabularnewline
~~&&&&(0.43***)&(0.43***)&(0.46***)&(0.48***)&(0.32***)&\tabularnewline
~~&&NKPC&&0.80***&0.77*&0.76&0.85&1.00&\tabularnewline
~~&&&&(0.12)&(0.11)&(0.08)&(-0.01)&(-0.01)&\tabularnewline
~~&&UCM &&1.07*&1.06*&1.06*&1.00&0.96&0.71\tabularnewline
~~&&&&(-0.35**)&(-0.34**)&(-0.34**)&(-0.27*)&(-0.24)&(0.14)\tabularnewline
\midrule
{\scshape Minnesota}&&&&&&&&&\tabularnewline
~~&1-step-ahead&FULL&&0.82**&0.82**&0.82**&0.82*&0.82**&\tabularnewline
~~&&&&(0.13)&(0.12)&(0.14)&(0.15)&(0.16*)&\tabularnewline
~~&&NKPC&&0.91&0.88&0.88*&0.95&1.08&\tabularnewline
~~&&&&(0.05)&(0.05)&(0.03)&(-0.04)&(-0.14)&\tabularnewline
~~&4-step-ahead&FULL&&0.61**&0.61**&0.62**&0.61**&0.61**&\tabularnewline
~~&&&&(0.36)&(0.37)&(0.37*)&(0.38*)&(0.37*)&\tabularnewline
~~&&NKPC&&0.81***&0.78***&0.78**&0.75&0.77&\tabularnewline
~~&&&&(0.13)&(0.12)&(0.12)&(0.06)&(0.03)&\tabularnewline
\bottomrule
\end{tabular}
\end{center}}
\begin{minipage}[c]{\linewidth}
\footnotesize{\textbf{Notes}: The table shows RMSEs with LPL's in parentheses below. Asterisks indicate statistical significance for each model relative to a random walk at the $1$ ($^{***}$), $5$ ($^{**}$) and $10$ ($^{*}$) percent significance levels. }
\end{minipage}
\end{table}

